DeepAuto: A Hierarchical Deep Learning Framework for Real-Time Prediction in Cellular Networks

Accurate real-time forecasting of key performance indicators (KPIs) is an essential requirement for various LTE/5G radio access network (RAN) automation. However, an accurate prediction can be very challenging in large-scale cellular environments due to complex spatio-temporal dynamics, network configuration changes and unavailability of real-time network data. In this work, we introduce a reusable analytics framework that enables real-time KPI prediction using a hierarchical deep learning architecture. Our prediction approach, namely DeepAuto, stacks multiple long short-term memory (LSTM) networks horizontally to capture instantaneous, periodic and seasonal patterns in KPI time-series. It further merge with feed-forward networks to learn the impact of network configurations and other external factors. We validate the approach by predicting two important KPIs, including cell load and radio channel quality, using large-scale real network streaming measurement data from the operator. For cell load prediction, DeepAuto model showed up to 15% improvement in Root Mean Square Error (RMSE) compared to naive method of using recent measurements for short-term horizon and up to 32% improvement for longer-term prediction.

==> pipeline.tex <==

\section{Real time prediction pipeline}
\label{production}
\begin{figure}[htbp]
\centerline{\includegraphics[scale=0.33]{figs/production_architecture.png}}
\caption{Analytics pipeline}
\label{pipeline}
\end{figure} 

Fig. \ref{pipeline} shows analytics pipeline of DeepAuto implementation for prediction. For training purposes, we use offline file-based data. 
Prediction phase uses real time Apache Kafka \cite{Narkhede:2017:KDG:3175825} feed from nationwide eNBs.
The prediction engine runs at every regional center close to each of the network management system (NMS) to reduce prediction latency. 
The kafka stream across multiple topics are correlated in real time and a time-series data will be generated for each of the cells. 
The model generated from the training phase is used to predict the future cells loads for next 1 min, 15 min and 1 hour at a granularity of 1 min. The results will be then fetched by various micro-services as needed to cater to various applications. The latency of real-time prediction is order of few seconds to enables various RAN automation use cases. 

